LOGO: A Long-Form Video Dataset for Group Action Quality Assessment

Action quality assessment (AQA) has become an emerging topic since it can be extensively applied in numerous scenarios. However, most existing methods and datasets focus on single-person short-sequence scenes, hindering the application of AQA in more complex situations. To address this issue, we construct a new multi-person long-form video dataset for action quality assessment named LOGO. Distinguished in scenario complexity, our dataset contains 200 videos from 26 artistic swimming events with 8 athletes in each sample along with an average duration of 204.2 seconds. As for richness in annotations, LOGO includes formation labels to depict group information of multiple athletes and detailed annotations on action procedures. Furthermore, we propose a simple yet effective method to model relations among athletes and reason about the potential temporal logic in long-form videos. Specifically, we design a group-aware attention module, which can be easily plugged into existing AQA methods, to enrich the clip-wise representations based on contextual group information. To benchmark LOGO, we systematically conduct investigations on the performance of several popular methods in AQA and action segmentation. The results reveal the challenges our dataset brings. Extensive experiments also show that our approach achieves state-of-the-art on the LOGO dataset. The dataset and code will be released at \url{https://github.com/shiyi-zh0408/LOGO }.

==> figures/action.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/action.png}
    \caption{Manual labeling logic circle diagram. The two inner circles represent the tech and free artistic swimming contest videos and the two outer ones mean the frame-wise labels. No free and required action labels respectively in the labels of tech and free videos. The formation labels only appear on the action its circle covers.}
    \label{fig:action}
\end{figure}

==> figures/actionsegmentation.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{imgs/actionsegmentation.png}
    \caption{Results for action segmentation using I3D and Br-Prompt features on LOGO. Parts of the actions are annotated on the color bar.}
    \label{fig:actionsegmentation}
\end{figure*}

==> figures/arg.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{imgs/ARG.png}
    \caption{The pipeline of Actor Relation Graphs for group activity recognition.}
    \label{fig:arg}
\end{figure}

==> figures/formation_detector.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/form_detector.png}
    \caption{An overview of our formation detector module (Take the number of anchors as 25 as an example). First, we split the picture into 25 patches and set the center point as the anchor for each patch. Next, we send the picture into a CNN and RoIAlign to extract features of each patch. Then we send the features added with positional embeddings into a self-attention module to find the contextual relations among patches. Finally, we use two fully-connected block to predict the confidence and relative coordinates respectively.}
    \label{fig:formationdetector}
\end{figure}

==> figures/label_instance.tex <==
\begin{figure}[h]
    \vspace{-0.3cm}
    \centering
    \setlength{\abovecaptionskip}{2cm}
    \includegraphics[width=1\linewidth]{imgs/label.png}
    \label{fig:label_ins}
    \vspace{-0.8cm}
\end{figure}

==> figures/multiangle.tex <==
\begin{figure}[h]
    \vspace{-0.8cm}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    \includegraphics[width=1\linewidth]{imgs/angle.png}
    \label{fig:angle}
    \vspace{-30pt}
\end{figure}

==> figures/segmentation.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{imgs/segmentation3.png}
    \caption{An visualization of our action segmentation experiments. \textbf{Acro.},  \textbf{Up.} and \textbf{Low.} represent \textit{Acrobatic, Upper and Lower movements}. \textbf{R1.}, \textbf{R2.} and \textbf{R3.} represents \textit{Required movements 1, 2 and 3}.}
    \label{fig:segmentation}
\end{figure*}

==> figures/sup_annotattion_tool.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/annotation-tool.png}
    \caption{Annotation tools. The top half is COIN annotation tool, and the lower half is Labelme.}
    \label{fig:supannotationtool}
\end{figure}

==> figures/sup_formationvisualization.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/sup_formation1.png}
    \caption{The additional visualizations of the prediction results of our formation detector method. The green polygons represent prediction results and the yellow polygons with blue edges are the ground truth. The results show that our approach can detect the positions of actors and distinguish whether the athlete is the formation vertex or not, which guarantees the reliability of the formation features.}
    \label{fig:supformationvisualization}
\end{figure*}

==> figures/teasor.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/overview15.png}
    \caption{An overview of the \textbf{\emph{LOGO}} dataset. LOGO is a multi-person long-form video dataset with frame-wise annotations on both action procedures (as shown in the second line) and formations (as shown in the third line, which reflects relations among actors) based on artistic swimming scenarios. It provides a potential for constructing an action quality assessment approach with the ability of modeling group information among actors. Longer video durations also challenge the ability of the method to aggregate long-term temporal information.}
    \label{fig:datasetoverview}
\end{figure*}

% \twocolumn[{
%     \renewcommand\twocolumn[1][]{#1}
%     % \maketitle
%     \begin{center}
%         \includegraphics[width=1\linewidth]{imgs/overview15.png}
%         \captionof{}
%         \label{fig:datasetoverview}
%     \end{center}
% }]

==> tables/aqa_SOTA_comparison.tex <==
\begin{table}[h]
\scriptsize
\vspace{-5pt}
\renewcommand\tabcolsep{2.2mm}
\label{table:aqasotacomparison}
\centering
\scalebox{0.75}{
\begin{tabular}{l|c|c|c|c}
\toprule
Dataset & MTL-AQA & AQA-7 & FineDiving & LOGO\\
\midrule
$\rho$ \uparrow / R-$\ell_2(\times100)$ \downarrow \textbf{CoRe} &0.9512 / 0.2600 &0.8401 / 2.12 &0.9061 / 0.3615 &\textcolor{red}{0.4712 / 5.4086} \\
$\rho$ \uparrow / R-$\ell_2(\times100)$ \downarrow \textbf{TPT} &0.9607 / 0.2378 &0.8715 / 1.68 &0.9182 / 0.3527 &\textcolor{red}{0.4732 / 5.3987} \\
\bottomrule
\end{tabular}}
\vspace{-14pt}
\end{table}

==> tables/aqawithas.tex <==
\begin{table}[h]
\vspace{-11pt}
\scriptsize
\renewcommand\tabcolsep{2.7mm}
\label{table:aqawithas}
\centering
\scalebox{0.75}{
\begin{tabular}{l|cc|cc}
\toprule
\multirow{}{}{Method} &\multicolumn{2}{c|}{I3D} & \multicolumn{2}{c}{SWIN}  \\
\cline{2-5}
& $\rho$ \uparrow & R-$\ell_2(\times100)$ \downarrow & $\rho$ \uparrow & R-$\ell_2(\times100)$ \downarrow\\
\midrule
USDL / \textbf{USDL+AS.} & 0.4259 / \textbf{0.4512} & 5.7364 / \textbf{4.8837} & 0.4725 / \textbf{0.5108} & 5.0762 / \textbf{5.0479} \\
CoRe / \textbf{CoRe+AS.} & 0.4712 / \textbf{0.4825} & 5.4086 / \textbf{5.2393} & 0.5002 / \textbf{0.5364} & 5.9597 / \textbf{4.9102} \\
TSA / \textbf{TSA+AS.} & 0.4518 / \textbf{0.4772} & 5.5326 / \textbf{5.4203} & 0.4751 / \textbf{0.4829} & 4.7778 / \textbf{5.3561} \\
\bottomrule
\end{tabular}}
\vspace{-13pt}
\end{table}

==> tables/arg.tex <==
\begin{table}[t]
\caption{Comparisons of AQA performance with ARG on LOGO. The higher $\rho$, the lower R-$\ell_2$, the better performance.}
\vspace{-5pt}
\footnotesize
\renewcommand\tabcolsep{6.8mm}
\label{table:arg}
\centering
\begin{tabular}{l|c|c}
\toprule
Method & $\rho$ \uparrow & R-$\ell_2(\times100)$ \downarrow \\
\midrule
ARG\cite{wu2019learning} & 0.3549 & 5.7778 \\
\midrule
USDL\cite{tang2020uncertainty}+GOAT & 0.4620 & 4.8739 \\
CoRe\cite{yu2021group}+GOAT & 0.4935 & 5.0716 \\
TSA\cite{xu2022finediving}+GOAT & 0.4855 & 5.3943 \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

==> tables/assota.tex <==
\begin{wraptable}{r}{4.8cm}
\scriptsize
% \renewcommand\arraystretch{1.4}
% \begin{center}
\setlength{\tabcolsep}{3pt}
\vspace{-12pt}
 \setlength{\tabcolsep}{0.8mm}{
 \scalebox{0.8}{
\begin{tabular}{l|l|ccc|c|c}
\toprule
Method & Features & \multicolumn{3}{c|}{F1@\{10,25,50\}} & Edit & Acc \\ 
\midrule
ASFormer & SWIN & 81.7 & 79.8 & 71.1 & 75.3 & 81.0 \\
ASFormer & I3D & 75.1 & 71.6 & 61.3 & 68.2 & 73.9 \\
ASFormer(GOAT) & SWIN & 82.2 & 80.3 & 73.6 & 75.9 & 81.7 \\
ASFormer(GOAT) & I3D & 75.8 & 72.0 & 62.1 & 68.8 & 74.6 \\
\bottomrule
\end{tabular}}}\label{table:asgoat}
\vspace{-12pt}
% \end{center}
\end{wraptable}

==> tables/computing_costs.tex <==
\begin{table}[t]
\caption{Comparisons of the inference time with existing AQA methods on LOGO.}
\vspace{-5pt}
\footnotesize
\renewcommand\tabcolsep{10.5mm}
\label{table:computingcosts}
\centering
\begin{tabular}{l|c}
\toprule
Method & Inference Time (s)\\
% \cline{2-5}
\midrule
USDL\cite{tang2020uncertainty} & 40.39 \\
USDL\cite{tang2020uncertainty}+GOAT & 40.40 \\
CoRe\cite{yu2021group} & 40.39 \\
CoRe\cite{yu2021group}+GOAT & 40.40 \\
TSA\cite{xu2022finediving} & 40.41 \\
TSA\cite{xu2022finediving}+GOAT & 40.51 \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

==> tables/exp.tex <==
\begin{table}[]
\small
\begin{center}
% \setlength{\tabcolsep}{5pt}
\caption{The action segmentation results of existing methods with GOAT on LOGO. \textit{+GOAT} indicates the method with GOAT.}
\vspace{-5pt}
\setlength{\tabcolsep}{0.9mm}{
\begin{tabular}{cc|cc}
\toprule
1 & 2 & 3 & 4 \\
\midrule
0.1 & 0.2 & 0.3 & 0.4 \\
\bottomrule
\end{tabular}}\label{table:example}
\vspace{-15pt}
\end{center}
\end{table}

==> tables/method22.tex <==
% \begin{table}[h]
% \vspace{-12pt}
% \scriptsize
% \renewcommand\tabcolsep{0.8mm}
% \label{table:method22}
% \centering
% \scalebox{0.75}{
% \begin{tabular}{l|cc}
% \toprule
% Method & $\rho$ \uparrow & R-$\ell_2(\times100)$ \downarrow\\
% \midrule
% TSA(CVPR 2022) & 0.4518 & 5.5326 \\
% TPT(ECCV 2022) & 0.4732 & 5.3987 \\
% TSA+GOAT & 0.4855 & 5.3943 \\
% TPT+GOAT & 0.4967 & 4.9535 \\
% \bottomrule
% \end{tabular}}
% \vspace{-15pt}
% \end{table}

\begin{table}[h]
\scriptsize
\vspace{-11pt}
\renewcommand\tabcolsep{2.2mm}
\label{table:aqasotacomparison}
\centering
\scalebox{0.75}{
\begin{tabular}{l|c|c|c|c}
\toprule
Method & TSA(CVPR 2022) & TPT(ECCV 2022) & TSA+GOAT & TPT+GOAT\\
\midrule
$\rho$ \uparrow / R-$\ell_2(\times100)$ \downarrow & 0.4518 / 5.5326 & 0.4732 / 5.3987 & 0.4855 / 5.3943 & 0.4967 / 4.9535 \\
\bottomrule
\end{tabular}}
\vspace{-12pt}
\end{table}

==> tables/ours2existingdataset.tex <==
% \begin{table}[h]
% \vspace{-12pt}
% \scriptsize
% \renewcommand\tabcolsep{0.8mm}
% \label{table:ours2existingdataset}
% \centering
% \scalebox{0.75}{
% \begin{tabular}{l|cc|cc}
% \toprule
% \multirow{Method} &\multicolumn{2}{c|}{Single} & \multicolumn{2}{c}{Syn.} \\
% \cline{2-5}
%  & $\rho$ \uparrow & R-$\ell_2(\times100)$ \downarrow & $\rho$ \uparrow & R-$\ell_2(\times100)$ \downarrow\\
% \midrule
% TSA (FineDiving) & 0.9332 & 0.3258 & 0.9146 & 0.3720\\
% TSA+GOAT (FineDiving) & - & - & 0.9276 & 0.3382 \\
% \midrule
% TPT (TASD-2) & - & - & 0.9314 & 0.7195\\
% TPT+GOAT (TASD-2) & - & - & 0.9462 & 0.6578\\
% \midrule
% TPT (AQA-7) & 0.8372 & 1.4328 & 0.9483 & 0.6861\\
% TPT+GOAT (AQA-7) & - & - & 0.9514 & 0.5823\\
% \bottomrule
% \end{tabular}}
% \vspace{-15pt}
% \end{table}

\begin{table}[h]
\scriptsize
\vspace{-11pt}
\renewcommand\tabcolsep{1.8mm}
\label{table:aqasotacomparison}
\centering
\scalebox{0.75}{
\begin{tabular}{l|c|c|c}
\toprule
Dataset & FineDiving (2 players) & TASD-2 (2 players) & AQA-7 (2 players) \\
\midrule
$\rho$ \uparrow / R-$\ell_2(\times100)$ \downarrow \textbf{TPT} & 0.9146 / 0.3720 & 0.9314 / 0.7195 & 0.9483 / 0.6861\\
$\rho$ \uparrow / R-$\ell_2(\times100)$ \downarrow \textbf{TPT+GOAT}& 0.9276 / 0.3382 & 0.9462 / 0.6578 & 0.9514 / 0.5823\\
\bottomrule
\end{tabular}}
\vspace{-12pt}
\end{table}

==> tables/rebuttal_dataset_comparison.tex <==
\begin{table}[h]
    % \centering
    \scriptsize
    \vspace{-20pt}
    \label{tab:rebuttal_action_set_comparison}
    \setlength{\tabcolsep}{0.8mm}{
    \scalebox{0.75}{\begin{tabular}{lccccccc}
    \toprule[1pt]
        Dataset & Duration & Avg.Dur. & Anno.Type & Samples & Events & Form.Anno. &Year\\ 
        \midrule
        FineGym & 161h,1m,45s & 45.7s & Action / Temp. Bound.& 12685 & 10 & \ding{55} & 2020\\
        Multisports & 18h,34m,40s & 20.9s & Action / Temp. Bound. / Spat. Local.& 3200 & 247& \ding{55} & 2021\\
    \midrule
        LOGO & 11h,20m,41s & 3m,24s & Action / Formation / Score & 200 & 26 & \ding{51}(15764) &\\
    \bottomrule[1pt]
    \end{tabular}}}
    \vspace{-13pt}
\end{table}

% \begin{table}[h]
% \scriptsize
% \vspace{-12pt}
% \renewcommand\tabcolsep{0.4mm}
% \label{table:aqasotacomparison}
% \centering
% \scalebox{0.75}{
% \begin{tabular}{l|c|c|c|c}
% \toprule
% Dataset & FineDiving (2 persons) & TPT(ECCV 2022) & TSA+GOAT & TPT+GOAT\\
% \midrule
% $\rho$ \uparrow / R-$\ell_2(\times100)$ \downarrow & 0.4518 / 5.5326 & 0.4732 / 5.3987 & 0.4855 / 5.3943 & 0.4967 / 4.9535 \\
% \bottomrule
% \end{tabular}}
% \vspace{-15pt}
% \end{table}
